SC-TPTP: An Extension of the TPTP Derivation Format for Sequent-Based Calculus

Motivated by the transfer of proofs between proof systems, and in particular from first order automated theorem provers (ATPs) to interactive theorem provers (ITPs), we specify an extension of the TPTP derivation text format to describe proofs in first-order logic: SC-TPTP. To avoid multiplication of standards, our proposed format over-specifies the TPTP derivation format by focusing on sequent formalisms. By doing so, it provides a high level of detail, is faithful to mathematical tradition, and cover multiple existing tools and in particular tableaux-based strategies. We make use of this format to allow the Lisa proof assistant to query the Go\'eland automated theorem prover, and implement a library of tools able to parse, print and check SC-TPTP proofs, export them into Coq files, and rebuild low-level proof steps from advanced ones.

==> figures/drinker_tptp.tex <==
% Proof of the \emph{drinker paradox} in \sctptp.

\begin{verbatim}
% SZS output start Proof for drinkers.p

fof(c_drinkers_p, conjecture, (? [X] : d(X) => (! [Y] : d(Y)))).

fof(f8, plain, {~(? [X] : d(X) => (! [Y] : d(Y))), 
~(d(X_0) => (! [Y] : d(Y))), d(X_0), ~(! [Y] : d(Y)), ~d(Sko_0), 
~(d(Sko_0) => (! [Y] : d(Y))), d(Sko_0)} --> {}, 
inference(leftHyp, [6, 4], [])).

fof(f7, plain, {~(? [X] : d(X) => (! [Y] : d(Y))), 
~(d(X_0) => (! [Y] : d(Y))), d(X_0), ~(! [Y] : d(Y)), ~d(Sko_0), 
~(d(Sko_0) => (! [Y] : d(Y)))} --> {}, inference(leftNotImp, [5], [f8])).

fof(f6, plain, {~(? [X] : d(X) => (! [Y] : d(Y))), 
~(d(X_0) => (! [Y] : d(Y))),  d(X_0), ~(! [Y] : d(Y)), ~d(Sko_0)} 
--> {}, inference(leftNotEx, [0, $fot(Sko_0)], [f7])).

fof(f5, plain, { ~(? [X] : d(X) => (! [Y] : d(Y))), 
~(d(X_0) => (! [Y] : d(Y))),  d(X_0),  ~(! [Y] : d(Y))} --> {}, 
inference(leftNotForall, [3, $fot(Sko_0)], [f6])).

fof(f4, plain, {~(? [X] : d(X) => (! [Y] : d(Y))), 
~(d(X_0) => (! [Y] : d(Y)))} --> {}, inference(leftNotImp, [1], [f5])).

fof(f3, plain, {~(? [X] : d(X) => (! [Y] : d(Y)))} --> {}, 
inference(leftNotEx, [0, $fot(X_0)], [f4])).

fof(f2, plain, {(? [X] : d(X) => (! [Y] : d(Y)))} --> 
{(? [X] : d(X) => (! [Y] : d(Y)))}, inference(hyp, [0, 0], [])).

fof(f1, plain, {} --> {(? [X] : d(X) => (! [Y] : d(Y))), 
~(? [X] : d(X) => (! [Y] : d(Y)))}, inference(rightNot, [1], [f2])).

fof(f0, plain, {} --> {(? [X] : d(X) => (! [Y] : d(Y)))}, 
inference(cut, [0], [f1, f3])).

% SZS output end Proof for drinkers.p
\end{verbatim}


==> figures/drinkers_coq.tex <==
\begin{figure}[h]
    \begin{lstlisting}[language=coq]
(* Add SCTPTP.p *)
    
Parameter sctptp_U : Set. (* universe *)
Parameter sctptp_I :  sctptp_U. (* an individual in the universe. *)

Parameter d: sctptp_U -> Prop.

Parameter X_0: sctptp_U.

Theorem drinker:  ~(~(exists (X: sctptp_U), (d(X) -> (forall (Y: sctptp_U), d(Y))))).
Proof.
intro H0.
(* [f3] *) apply H0. exists X_0. apply NNPP. intros H1. 
(* [f4] *) apply (leftNotImp  _  _  H1). intros H2 H3.
(* [f5] *) apply H3. intros Sko_0_15. apply NNPP. intros  H4. 
(* [f6] *) apply H0. exists Sko_0_15. apply NNPP. intros H5. 
(* [f7] *) apply (leftNotImp  _  _  H5). intros H6 H7.
(* [f8] *) auto.
Qed.
    \end{lstlisting}
    \caption{Proof of the \emph{drinker paradox} in \coq{} outputted by our tool.}
    \label{fig:drinker_coq}
\end{figure}


==> figures/format_description.tex <==
\begin{table}
    \centering
    \begin{tabular}{|c|c|c|}
         \hline
         Element & Definition & Type\\ \hline
         \texttt{id\_step} & identifier of the sequent step & string (must start by a letter) \\ \hline
         \texttt{premises} & list of the premises of the sequent step & string list \\ \hline
         \texttt{conclusions} & list of the conclusions of the sequent step & string list \\ \hline
         \texttt{rule\_name} & the rule applied at this step & string (must be in the list of table~\ref{tab:param_data})  \\ \hline
         \texttt{parameters\_list} & \makecell{list of parameters corresponding to\\a specific rule (see table~\ref{tab:param_data})} & strings, integers, anything allowed by TPTP (\$fot) \\ \hline
         \texttt{id\_parent} & \makecell{identifier of the parent(s) of\\the current sequent step} & string (must refer to other \texttt{id\_step})  \\ \hline
     \end{tabular}
    \caption{Inference rules data}
    \label{tab:inference_rules_datas}
\end{table}

==> figures/gs3.tex <==
\begin{figure}[ht]
  \alwaysRootAtBottom
  \framebox[\textwidth]{
    \parbox{\textwidth}{
      \begin{subfigure}{\textwidth}
        \begin{minipage}{.24\linewidth}
          \begin{prooftree}
            \AXC{}
            \RL{ax}
            \UICm{\Delta, \bot \vdash}
          \end{prooftree}
        \end{minipage}
        \begin{minipage}{.24\linewidth}
          \begin{prooftree}
            \AXC{}
            \RL{ax}
            \UICm{\Delta, \neg\top \vdash}
          \end{prooftree}
        \end{minipage}
        \begin{minipage}{.24\linewidth}
          \begin{prooftree}
            \AXC{}
            \RL{ax}
            \UICm{\Delta, P, \neg P \vdash}
          \end{prooftree}
        \end{minipage}
        \begin{minipage}{.24\linewidth}
          \begin{prooftree}
            \AXCm{\Delta \vdash}
            \RL{w}
            \UICm{\Delta, P \vdash}
          \end{prooftree}
        \end{minipage}
        \caption{Structural and axiomatic rules.}
      \end{subfigure}

      \bigskip
      
      \begin{subfigure}{\textwidth}
        \centering
        \begin{minipage}{.45\linewidth}
          \begin{prooftree}
            \AXCm{\Delta, \neg\neg P, P \vdash}
            \RLm{\neg_\neg}
            \UICm{\Delta, \neg\neg P \vdash}
          \end{prooftree}
        \end{minipage}
        \begin{minipage}{.45\linewidth}
          \begin{prooftree}
            \AXCm{\Delta, P \land Q, P, Q \vdash}
            \RLm{\land}
            \UICm{\Delta, P \land Q \vdash}
          \end{prooftree}
        \end{minipage}

        \medskip

        \begin{minipage}{.45\linewidth}
          \begin{prooftree}
            \AXCm{\Delta, \neg(P\lor Q), \neg P, \neg Q \vdash}
            \RLm{\neg_\lor}
            \UICm{\Delta, \neg(P\lor Q) \vdash}
          \end{prooftree}
        \end{minipage}
        \begin{minipage}{.45\linewidth}
          \begin{prooftree}
            \AXCm{\Delta, \neg(P \Rightarrow Q), P, \neg Q \vdash}
            \RLm{\neg_\Rightarrow}
            \UICm{\Delta, \neg(P \Rightarrow Q) \vdash}
          \end{prooftree}
        \end{minipage}
        \caption{Non-branching propositional rules.}
      \end{subfigure}

      \bigskip

      \begin{subfigure}{\textwidth}
        \begin{minipage}{.45\linewidth}
          \begin{prooftree}
            \AXCm{\Delta, P \lor Q, P \vdash}
            \AXCm{\Delta, P \lor Q, Q \vdash}
            \RLm{\lor}
            \BICm{\Delta, P \lor Q \vdash}
          \end{prooftree}
        \end{minipage}
        \begin{minipage}{.5\linewidth}
          \begin{prooftree}
            \AXCm{\Delta, P \Rightarrow Q, \neg P \vdash}
            \AXCm{\Delta, P \Rightarrow Q, Q \vdash}
            \RLm{\Rightarrow}
            \BICm{\Delta, P \Rightarrow Q\vdash}
          \end{prooftree}
        \end{minipage}\hfill
        
        \medskip

        \begin{minipage}{\linewidth}
          \begin{prooftree}
            \AXCm{\Delta, \neg(P\land Q), \neg P \vdash}
            \AXCm{\Delta, \neg(P\land Q), \neg Q \vdash}
            \RLm{\neg_\land}
            \BICm{\Delta, \neg(P \land Q) \vdash}
          \end{prooftree}
        \end{minipage}

        \medskip

        \begin{minipage}{\linewidth}
          \begin{prooftree}
            \AXCm{\Delta, P \Leftrightarrow Q, \neg P, \neg Q \vdash}
            \AXCm{\Delta, P \Leftrightarrow Q, P, Q \vdash}
            \RLm{\Leftrightarrow}
            \BICm{\Delta, P \Leftrightarrow Q \vdash}
          \end{prooftree}
        \end{minipage}

        \medskip

        \begin{minipage}{\linewidth}
          \begin{prooftree}
            \AXCm{\Delta, \neg(P \Leftrightarrow Q), P, \neg Q \vdash}
            \AXCm{\Delta, \neg(P \Leftrightarrow Q), \neg P, Q \vdash}
            \RLm{\neg_\Leftrightarrow}
            \BICm{\Delta, \neg(P \Leftrightarrow Q) \vdash}
          \end{prooftree}
        \end{minipage}
        \caption{Branching propositional rules.}
      \end{subfigure}

      \bigskip

      \begin{subfigure}{\textwidth}
        \begin{minipage}{.5\linewidth}
          \begin{prooftree}
            \AXCm{\Delta, \exists x \; P, P[x \mapsto c] \vdash}
            \RLm{\exists}
            \UICm{\Delta, \exists x \; P \vdash}            
          \end{prooftree}
        \end{minipage}
        \begin{minipage}{.5\linewidth}
          \begin{prooftree}
            \AXCm{\Delta, \neg\forall x \; P, \neg P[x \mapsto c] \vdash}
            \RLm{\neg_\forall}
            \UICm{\Delta, \neg\forall x \; P \vdash}
          \end{prooftree}
        \end{minipage}
        \caption{Skolemization rules, where $c$ is a fresh constant.}
      \end{subfigure}

      \bigskip

      \begin{subfigure}{\textwidth}
        \begin{minipage}{.5\linewidth}
          \begin{prooftree}
            \AXCm{\Delta, \forall x \; P, P[x \mapsto t] \vdash}
            \RLm{\forall}
            \UICm{\Delta, \forall x \; P \vdash}
          \end{prooftree}
        \end{minipage}
        \begin{minipage}{.5\linewidth}
          \begin{prooftree}
            \AXCm{\Delta, \neg\exists x \; P, \neg P[x\mapsto t] \vdash}
            \RLm{\neg_\exists}
            \UICm{\Delta, \neg\exists x \; P \vdash}
          \end{prooftree}
        \end{minipage}
        \caption{Instantiation rules, where $t$ is a ground term.}
      \end{subfigure}

            \bigskip

      \begin{subfigure}{\textwidth}
      \begin{minipage}{.5\linewidth}
            \begin{prooftree}
            \AXCm{\Delta, s = t, P[t] \vdash}
            \RLm{=_1}
            \UICm{\Delta, s = t, P[s] \vdash}
          \end{prooftree}
      \end{minipage}%
      \begin{minipage}{.5\linewidth}
            \begin{prooftree}
            \AXCm{\Delta, s = t, P[s] \vdash}
            \RLm{=_2}
            \UICm{\Delta, s = t, P[t] \vdash}
          \end{prooftree}
      \end{minipage}
        \caption{Equality rules, where $s$ and $t$ are ground terms.}
      \end{subfigure}
    }}
    \caption{Rules of the \gs{} calculus.}
    \label{fig:rulesGS3}
    \alwaysRootAtTop
\end{figure} 

==> figures/tableaux.tex <==
\begin{figure}[ht]
    \begin{center}
        \framebox[\textwidth]{
            \parbox{\textwidth}{
                \begin{subfigure}{\textwidth}
                    \begin{minipage}{.33\textwidth}
                        \begin{prooftree}
                            \rootAtTop
                            \AXCm{\odot}
                            \RLm{\odot_\bot}
                            \UICm{\bot}
                        \end{prooftree}
                    \end{minipage}\hfill
                    \begin{minipage}{.33\textwidth}
                        \begin{prooftree}
                            \rootAtTop
                            \AXCm{\odot}
                            \RLm{\odot_{\neg\top}}
                            \UICm{\neg\top}
                        \end{prooftree}
                    \end{minipage}\hfill
                    \begin{minipage}{.33\textwidth}
                        \begin{prooftree}
                            \rootAtTop
                            \AXCm{\sigma}
                            \RLm{\odot_\sigma, P\sigma = Q\sigma}
                            \UICm{P, \neg Q}
                        \end{prooftree}
                    \end{minipage}
                    \caption{$\odot$ rules.}
                \end{subfigure}
                
                \vspace{.2cm}

                \begin{subfigure}{\textwidth}
                    \begin{minipage}{.2\textwidth}
                        \begin{prooftree}
                            \rootAtTop
                            \AXCm{P}
                            \RLm{\alpha_{\neg\neg}}
                            \UICm{\neg\neg P}
                        \end{prooftree}
                    \end{minipage}\hfill
                    \begin{minipage}{.2\textwidth}
                        \begin{prooftree}
                            \rootAtTop
                            \AXCm{P, Q}
                            \RLm{\alpha_{\land}}
                            \UICm{P \land Q}
                        \end{prooftree}
                    \end{minipage}\hfill
                    \begin{minipage}{.2\textwidth}
                        \begin{prooftree}
                            \rootAtTop
                            \AXCm{\neg P, \neg Q}
                            \RLm{\alpha_{\neg\lor}}
                            \UICm{\neg(P \lor Q)}
                        \end{prooftree}
                    \end{minipage}\hfill
                    \begin{minipage}{.2\textwidth}
                        \begin{prooftree}
                            \rootAtTop
                            \AXCm{P, \neg Q}
                            \RLm{\alpha_{\neg\Rightarrow}}
                            \UICm{\neg(P \Rightarrow Q)}
                        \end{prooftree}
                    \end{minipage}\hfill
                    \caption{$\alpha$ rules.}
                \end{subfigure}

                \vspace{.2cm}

                \begin{subfigure}{\textwidth}
                    \begin{minipage}{.33\textwidth}
                        \begin{prooftree}
                            \rootAtTop
                            \AXCm{P}
                            \AXCm{Q}
                            \RLm{\beta_{\lor}}
                            \BICm{P \lor Q}
                        \end{prooftree}
                    \end{minipage}
                    \begin{minipage}{.33\textwidth}
                        \begin{prooftree}
                            \rootAtTop
                            \AXCm{\neg P}
                            \AXCm{Q}
                            \RLm{\beta_{\Rightarrow}}
                            \BICm{P \Rightarrow Q}
                        \end{prooftree}
                    \end{minipage}
                    \begin{minipage}{.33\textwidth}
                        \begin{prooftree}
                            \rootAtTop
                            \AXCm{\neg P}
                            \AXCm{\neg Q}
                            \RLm{\beta_{\neg\land}}
                            \BICm{\neg(P \land Q)}
                        \end{prooftree}
                    \end{minipage}

                    \hfill
                    \begin{minipage}{.4\textwidth}
                        \begin{prooftree}
                            \rootAtTop
                            \AXCm{\neg P, \neg Q}
                            \AXCm{P, Q}
                            \RLm{\beta_\Leftrightarrow}
                            \BICm{P \Leftrightarrow Q}
                        \end{prooftree}
                    \end{minipage}
                    \begin{minipage}{.5\textwidth}
                        \begin{prooftree}
                            \rootAtTop
                            \AXCm{P, \neg Q}
                            \AXCm{\neg P, Q}
                            \RLm{\beta_{\neg\Leftrightarrow}}
                            \BICm{\neg(P \Leftrightarrow Q)}
                        \end{prooftree}
                    \end{minipage}
                    \caption{$\beta$ rules.}
                \end{subfigure}

                \vspace{.2cm}

                \begin{subfigure}{\textwidth}
                    \begin{minipage}{.45\textwidth}
                        \begin{prooftree}
                            \rootAtTop
                            \AXCm{P[x \mapsto c]}
                            \RLm{\delta_{\exists}}
                            \UICm{\exists x.\,P}
                        \end{prooftree}
                    \end{minipage}\hfill
                    \begin{minipage}{.45\textwidth}
                        \begin{prooftree}
                            \rootAtTop
                            \AXCm{\neg P[x \mapsto c]}
                            \RLm{\delta_{\neg\forall}}
                            \UICm{\neg\forall x.\,P}
                        \end{prooftree}
                    \end{minipage}

                    \caption{$\delta$ rules, where c is a fresh constant.}
                \end{subfigure}

                \vspace{.2cm}

                \begin{subfigure}{\textwidth}
                    \begin{minipage}{.45\textwidth}
                        \begin{prooftree}
                            \rootAtTop
                            \AXCm{P[x \mapsto t]}
                            \RLm{\gamma_{\forall}}
                            \UICm{\forall x.\,P}
                        \end{prooftree}
                    \end{minipage}\hfill
                    \begin{minipage}{.45\textwidth}
                        \begin{prooftree}
                            \rootAtTop
                            \AXCm{\neg P[x \mapsto t]}
                            \RLm{\gamma_{\neg\exists}}
                            \UICm{\neg\exists x.\,P}
                        \end{prooftree}
                    \end{minipage}

                    \caption{$\gamma$ rules, where $t$ is a ground term.}
                \end{subfigure}

                \vspace{.2cm}

                \begin{subfigure}{\textwidth}
                \begin{minipage}{.5\textwidth}
                        \begin{prooftree}
                            \rootAtTop
                            \AXCm{s = t, P[t]}
                            \RLm{=_1}
                            \UICm{s = t, P[s]}
                        \end{prooftree}
                \end{minipage}%
                \begin{minipage}{.5\textwidth}
                        \begin{prooftree}
                            \rootAtTop
                            \AXCm{s = t, P[s]}
                            \RLm{=_2}
                            \UICm{s = t, P[t]}
                        \end{prooftree}
                \end{minipage}
                    \caption{Equality rule, where $s$ and $t$ are ground terms.}
                \end{subfigure}
                
        }}
    \end{center}
    \caption{Rules of the free-variable tableau calculus. Note that the rules are written in the opposite direction as in \autoref{fig:deduct_rules_1}. This emphasizes the proof search nature of tableau: to prove the upper part of a deduction rule, it is sufficient to prove the bottom part of the deduction rule.}
    \label{fig:rulesTableau}
  \end{figure}

==> figures/tfx.tex <==
 \begin{figure}[tbhp]
        \parbox{\textwidth}{
            \begin{align*}
                \texttt{<tff\_annotated>} ::= & \qquad \texttt{tff(<name>, <formula\_role>, <tff\_formula>, <annotations>).}            \\
                \texttt{<formula\_role>} ::= & \qquad \texttt{assumption | axiom | conjecture | plain}  \\ 
                \texttt{<tff\_formula>} ::= & \qquad \texttt{<tff\_logical\_formula>}  \mid \texttt{<tff\_atom\_typing>}  \mid \texttt{<tff\_subtypes>}  \\ 
                
                \texttt{<tfx\_sequent>} ::= & \qquad \texttt{<tfx\_tuple>  \texttt{-->}  <tfx\_tuple>}                        \\
                \texttt{<tfx\_tuple>} ::= & \qquad \texttt{[]} \;  \mid  \texttt{ [<tff\_arguments>] }                      \\
                \texttt{<tff\_arguments>} ::= & \qquad \texttt{ <tff\_term> }  \mid \texttt{ <tff\_term>, <tff\_arguments> } \\
                \texttt{<tff\_term>} ::= & \qquad \texttt{ <tff\_logic\_formula> }  \mid \texttt{ <defined\_term> } \mid \texttt{ <tfx\_tuple> } \\
            \end{align*}}
    \caption{Main elements of the \sctptp{} syntax. \texttt{logic\_formula} is the FOF syntax for logical formulas and  \texttt{defined\_terms} a set of predfined elements (sych as numbers of special characters). For \sctptp{} derivations, annotations are of the form \texttt{inference(rule, [parameters], [premises])}.}
    \label{fig:fofx}
\end{figure}

==> figures/two_sided_sc.tex <==
\begin{figure}[hp]
      \begin{center}
        \begin{tabular}{|l l|}
          \hline
          & \vspace*{-1ex}\\
          \AxiomC{}
          \RightLabel{\texttt{ hyp}}
          \UnaryInfC{$\Gamma, \phi \vdash \phi, \Delta$}
          \DisplayProof &
          \AxiomC{$\Gamma \vdash \phi, \Delta$}
          \AxiomC{$\Sigma, \phi \vdash \Pi$}
          \RightLabel{\texttt{ cut}}
          \BinaryInfC{$\Gamma, \Sigma \vdash \Delta, \Pi$}
          \DisplayProof
          \\[4.5ex]

          \AxiomC{$\Gamma \vdash \Delta$}
          \RightLabel{\texttt{ leftWeaken}}
          \UnaryInfC{$\Gamma, \phi \vdash \Delta$}
          \DisplayProof &
          \AxiomC{$\Gamma \vdash \Delta$}
          \RightLabel{\texttt{ rightWeaken}}
          \UnaryInfC{$\Gamma \vdash \phi, \Delta$}
          \DisplayProof
          \\[4.5ex]
          \hline
          & \vspace*{-1ex}\\

        & \vspace*{-1ex}\\
          \AxiomC{}
          \RightLabel{\texttt{ refl}}
          \UnaryInfC{$\Gamma, \vdash s = s, \Delta$}
          \DisplayProof &
          \\[4.5ex]

          \AxiomC{$\Gamma, s = t, \phi[t] \vdash \Delta$}
          \RightLabel{\texttt{ leftSubst}}
          \UnaryInfC{$\Gamma, s = t, \phi[s] \vdash \Delta$}
          \DisplayProof &
          \AxiomC{$\Gamma, s = t \vdash \phi[t], \Delta$}
          \RightLabel{\texttt{ rightSubst}}
          \UnaryInfC{$\Gamma, s = t \vdash \phi[s], \Delta$}
          \DisplayProof
          \\[4.5ex]
          \hline
          & \vspace*{-1ex}\\

          \AxiomC{$\Gamma, \phi, \psi \vdash \Delta$}
          \RightLabel{\texttt{ leftAnd}}
          \UnaryInfC{$\Gamma, \phi \land \psi \vdash \Delta$}
          \DisplayProof &
          \AxiomC{$\Gamma, \phi \vdash \Delta$}
          \AxiomC{$\Sigma, \psi \vdash \Pi$}
          \RightLabel{\texttt{ leftOr}}
          \BinaryInfC{$\Gamma, \Sigma, \phi\lor \psi \vdash \Delta, \Pi$}
          \DisplayProof 
          \\[4.5ex]

          \AxiomC{$\Gamma \vdash \phi, \Delta$}
          \AxiomC{$\Sigma, \psi \vdash \Pi$}
          \RightLabel{\texttt{ leftImp}}
          \BinaryInfC{$\Gamma, \Sigma, \phi\Rightarrow \psi \vdash \Delta, \Pi$}
          \DisplayProof &
          \\[4.5ex]

          \AxiomC{$\Gamma, \phi \Rightarrow \psi, \psi \Rightarrow \phi \vdash \Delta$}
          \RightLabel{\texttt{ leftIff}}
          \UnaryInfC{$\Gamma, \phi \Leftrightarrow \psi \vdash \Delta$}
          \DisplayProof &
          \AxiomC{$\Gamma \vdash \phi, \Delta$}
          \RightLabel{\texttt{ leftNot}}
          \UnaryInfC{$\Gamma, \neg \phi \vdash \Delta$}
          \DisplayProof 
          \\[4.5ex]

          \AxiomC{$\Gamma, \phi[x := t] \vdash \Delta$}
          \RightLabel{\texttt{ leftAll}}
          \UnaryInfC{$\Gamma, \forall x. \phi  \vdash \Delta$}
          \DisplayProof &          
          \AxiomC{$\Gamma, \phi \vdash \Delta$}
          \RightLabel{\texttt{ leftEx}}
          \UnaryInfC{$\Gamma, \exists x. \phi \vdash \Delta$}
          \DisplayProof
          \\[4.5ex]
          \hline
           & \vspace*{-1ex}\\

          
          \AxiomC{$\Gamma \vdash \phi, \Delta$}
          \AxiomC{$\Sigma \vdash \psi, \Pi$}
          \RightLabel{\texttt{ rightAnd}}
          \BinaryInfC{$\Gamma, \Sigma \vdash \phi \land \psi,  \Delta, \Pi$}
          \DisplayProof &
          \AxiomC{$\Gamma \vdash \phi, \psi \Delta$}
          \RightLabel{\texttt{ rightOr}}
          \UnaryInfC{$\Gamma \vdash \phi \lor \psi,  \Delta$}
          \DisplayProof
          \\[4.5ex]


          \AxiomC{$\Gamma \phi \vdash \psi, \Delta$}
          \RightLabel{\texttt{ rightImp}}
          \UnaryInfC{$\Gamma \vdash \phi \Rightarrow \psi,  \Delta$}
          \DisplayProof &
          \\[4.5ex]

          \AxiomC{$\Gamma \vdash \phi \Rightarrow \psi, \Delta$}
          \AxiomC{$\Sigma \vdash \psi \Rightarrow \phi, \Pi$}
          \RightLabel{\texttt{ rightIff}}
          \BinaryInfC{$\Gamma, \Sigma \vdash \phi \Leftrightarrow \psi,  \Delta, \Pi$}
          \DisplayProof
          &
          \AxiomC{$\Gamma, \phi \vdash \Delta$}
          \RightLabel{\texttt{ rightNot}}
          \UnaryInfC{$\Gamma \vdash \neg \phi ,  \Delta$}
          \DisplayProof
          \\[4.5ex]

          \AxiomC{$\Gamma \vdash \phi, \Delta$}
          \RightLabel{\texttt{ rightAll}}
          \UnaryInfC{$\Gamma \vdash \forall x. \phi,  \Delta$}
          \DisplayProof &
          \AxiomC{$\Gamma \vdash \phi[x := t], \Delta$}
          \RightLabel{\texttt{ rightEx}}
          \UnaryInfC{$\Gamma \vdash \exists x. \phi,  \Delta$}
          \DisplayProof
          \\[4.5ex]
          \hline
          %& \\[1ex]
        \end{tabular}
      \end{center}
  \caption{Semantics of the deduction rules of proof steps of classical two-sided and one-sided sequent calculus.}
  \label{fig:deduct_rules_1}
\end{figure}
